Codes, Cubes, and Graphical Designs

Graphical designs are an extension of spherical designs to functions on graphs. We connect linear codes to graphical designs on cube graphs, and show that the Hamming code in particular is a highly effective graphical design. We show that even in highly structured graphs, graphical designs are distinct from the related concepts of extremal designs, maximum stable sets in distance graphs, and $t$-designs on association schemes.

==> CatherinesDefns.tex <==
%Blackboard Bold


\def\AA{{\mathbb A}}
\def\CC{{\mathbb C}} 
\def\DD{{\mathbb D}} 
\def\EE{{\mathbb E}}
\def\FF{{\mathbb F}}
\def\GG{{\mathbb G}}
\def\HH{{\mathbb H}}
\def\II{{\mathbb I}}
\def\JJ{{\mathbb J}}
\def\KK{{\mathbb K}}
\def\MM{{\mathbb M}}
\def\NN{{\mathbb N}}
\def\OO{{\mathbb O}}
\def\PP{{\mathbb P}}
\def\QQ{{\mathbb Q}}
\def\RR{{\mathbb R}}
\def\SS{{\mathbb S}}
\def\TT{{\mathbb T}}
\def\VV{{\mathbb V}}
\def\XX{{\mathbb X}}
\def\ZZ{{\mathbb Z}}


%Italic
\def\cal{\mathcal}
\def\cA{{\cal A}}
\def\cB{{\cal B}}
\def\cC{{\cal C}}
\def\cD{{\cal D}}
\def\cE{{\cal E}}
\def\cF{{\cal F}}
\def\cG{{\cal G}}
\def\cH{{\cal H}}
\def\cI{{\cal I}}
\def\cJ{{\cal J}}
\def\cK{{\cal K}}
\def\cL{{\cal L}}
\def\cM{{\cal M}}
\def\cN{{\cal N}}
\def\cO{{\cal O}}
\def\cP{{\cal P}}
\def\cQ{{\cal Q}}
\def\cR{{\cal R}}
\def\cS{{\cal S}}
\def\cT{{\cal T}}
\def\cU{{\cal U}}
\def\cV{{\cal V}}
\def\cW{{\cal W}}
\def\cX{{\cal X}}
\def\cY{{\cal Y}}
\def\cZ{{\cal Z}}

%Greek
\def\a{\alpha}
\def\b{\beta}
\def\c{\gamma}
\def\d{\delta}
\def\e{\varepsilon}
\def\g{\gamma}
\def\l{\lambda}
\def\L{\Lambda}
\def\o{\omega}
\def\s{\sigma}
\def\t{\tau}
\renewcommand{\phi}{\varphi}

%emptyset
\def\vn{\varnothing}

%fat numbers
\def\ones{\mathbbm{1}}
\def\zeros{\mathbf{0} }

%asterisk numbers
\def\xopt{x^*}
\def\yopt{y^*}
\def\Xopt{X^*}

%operator names 
\def\Aff{\operatorname {Aff}}
\def\conv{\operatorname {conv}}
\def\cl{\operatorname {cl}}
\def\interior{\operatorname {int}}
\def\supp{\operatorname {supp}}
\def\Tr{\operatorname {Tr}}
\def\rk{\operatorname {rk}}
\def\Diag{\operatorname {Diag}}
\def\Vert{\operatorname {Vert}}
\def\proj{\operatorname {proj}}
\def\spanset{\operatorname {span}}
\def\col{\operatorname {col}}
\def\row{\operatorname {row}}
\def\design{\operatorname {design}}
\def\dist{\operatorname {dist}}
\def\eff{\operatorname {efficacy}}
%lefts and rights
\def\lang{\left\langle}
\def\rang{\right\rangle}
\def\lnorm{\left\|}
\def\rnorm{\right\|}
\def\labs{\left|}
\def\rabs{\right|}


